ForgeryNet: A Versatile Benchmark for Comprehensive Forgery Analysis

The rapid progress of photorealistic synthesis techniques has reached at a critical point where the boundary between real and manipulated images starts to blur. Thus, benchmarking and advancing digital forgery analysis have become a pressing issue. However, existing face forgery datasets either have limited diversity or only support coarse-grained analysis. To counter this emerging threat, we construct the ForgeryNet dataset, an extremely large face forgery dataset with unified annotations in image- and video-level data across four tasks: 1) Image Forgery Classification, including two-way (real / fake), three-way (real / fake with identity-replaced forgery approaches / fake with identity-remained forgery approaches), and n-way (real and 15 respective forgery approaches) classification. 2) Spatial Forgery Localization, which segments the manipulated area of fake images compared to their corresponding source real images. 3) Video Forgery Classification, which re-defines the video-level forgery classification with manipulated frames in random positions. This task is important because attackers in real world are free to manipulate any target frame. and 4) Temporal Forgery Localization, to localize the temporal segments which are manipulated. ForgeryNet is by far the largest publicly available deep face forgery dataset in terms of data-scale (2.9 million images, 221,247 videos), manipulations (7 image-level approaches, 8 video-level approaches), perturbations (36 independent and more mixed perturbations) and annotations (6.3 million classification labels, 2.9 million manipulated area annotations and 221,247 temporal forgery segment labels). We perform extensive benchmarking and studies of existing face forensics methods and obtain several valuable observations.

==> 1619_sup.tex <==
% % This version of CVPR template is provided by Ming-Ming Cheng.
% % Please leave an issue if you found a bug:
% % https://github.com/MCG-NKU/CVPR_Template.

% \documentclass[review]{cvpr}
% %\documentclass[final]{cvpr}

% \usepackage{cite}
% \usepackage{float}
% \usepackage{times}
% \usepackage{epsfig}
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage{mmstyles}
% \usepackage{multirow}
% \usepackage{caption}
% \usepackage{rotating}

% \usepackage{array}
% \makeatletter
% \def\hlinew#1{%
%   \noalign{\ifnum0=`}\fi\hrule \@height #1 \futurelet
%   \reserved@a\@xhline}
% \makeatother

% \usepackage{makecell}

% % add table def by gjyin
% \newcolumntype{P}[1]{>{\raggedright\arraybackslash}p{#1}}
% \newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}

% % Include other packages here, before hyperref.
% \newcommand{\reff}[1]{\textcolor{red}{[ref#1]}}
% \newcommand{\name}[1]{ForgeryNet}
% \newcommand{\jshao}[1]{\textcolor[rgb]{1,0.5,0}{[jshao -- #1]}}
% \newcommand{\gjyin}[1]{\textcolor[rgb]{1,0.5,1}{[gjyin -- #1]}}
% \newcommand{\ynhe}[1]{\textcolor[rgb]{0.5,0,0.5}{[ynhe -- #1]}}
% \newcommand{\bgan}[1]{\textcolor[rgb]{0,0.5,0.5}{[bgan -- #1]}}
% \newcommand{\lsheng}[1]{\textcolor[rgb]{0,0,0.5}{[lsheng -- #1]}}
% \newcommand{\ycz}[1]{\textcolor{red}{#1}}
% \newcommand{\zyc}[1]{\textcolor[rgb]{0.3,0.6,0.9}{[zyc -- #1]}}

% \usepackage{xr-hyper}
% \makeatletter
% \newcommand*{\addFileDependency}[1]{% argument=file name and extension
%   \typeout{(#1)}
%   \@addtofilelist{#1}
%   \IfFileExists{#1}{}{\typeout{No file #1.}}
% }
% \makeatother

% \newcommand*{\myexternaldocument}[1]{%
%     \externaldocument{#1}%
%     \addFileDependency{#1.tex}%
%     \addFileDependency{#1.aux}%
% }
% \myexternaldocument{1619main}

% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \usepackage[pagebackref=true,breaklinks=true,colorlinks,bookmarks=false]{hyperref}


% \def\cvprPaperID{1619} % *** Enter the CVPR Paper ID here
% \def\confYear{CVPR 2021}
% %\setcounter{page}{4321} % For final version only


% \begin{document}

% %%%%%%%%% TITLE
% \title{ForgeryNet: A Versatile Benchmark for Comprehensive Forgery Analysis
% (Supplementary Material)}

% \author{First Author\\
% Institution1\\
% Institution1 address\\
% {\tt\small firstauthor@i1.org}
% % For a paper whose authors are all at the same institution,
% % omit the following lines up until the closing ``}''.
% % Additional authors and addresses can be added with ``\and'',
% % just like the second author.
% % To save space, use either the email address or home page, not both
% \and
% Second Author\\
% Institution2\\
% First line of institution2 address\\
% {\tt\small secondauthor@i2.org}
% }

% \maketitle
% \appendix
% %%%%%%%%% BODY TEXT
% \input{appendix/a_original_data}
% \input{appendix/b_pre_process}
% \input{appendix/c_forgery_approach}
% \input{appendix/d_re_rendering}
% \input{appendix/e_perturbation}
% \input{appendix/f_annotation}
% \input{appendix/g_dataset_split}
% \input{appendix/h_benchmark}

% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% }

% \end{document}

